De-meaning Simulation Studies

In simulation studies evaluating asymptotic approximations it is common practice to report averages and standard deviations over repeated simulations. We argue that quantile-based summaries are more appropriate from both a theoretical and practical point of view. Theoretically, convergence of moments -- or even existence of moments -- is not guaranteed by convergence in distribution, so sample moments are not ideal for assessing the accuracy of a distributional approximation. In practice, means and variances are not good summaries of approximately-Normal distributions that may have occasional outliers. We suggest the median and median absolute deviation, and empirical confidence interval coverage, as better general summaries, and argue that moments should be reserved for simulation settings where they are of substantive interest.

==> synthetic_simulation_results_cOR_n10000.tex <==
\begin{table}[!h]
\centering
\caption{Estimating the cOR in a rare-outcome, high missing-data setting, n = 10000.\label{tab:synthetic_results_cOR_n10000}}
\centering
\fontsize{8.5}{10.5}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{l>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}}
\toprule
Est & Mn bias & \textbf{Med bias} & WMn bias & TMn bias & ESE & \textbf{MAD} & Mean ASE & \textbf{Med ASE} & WMn ASE & TMn ASE & bias / SE & CP & \textbf{CP*}\\
\midrule
GR & -0.16 & 0.01 & -0.02 & -0.01 & 2.58 & 0.41 & 0.36 & 0.33 & 0.35 & 0.34 & 0.03 & 0.72 & 0.86\\
IPW & -0.33 & -0.08 & -0.13 & -0.11 & 3.49 & 1.03 & 0.87 & 0.83 & 0.86 & 0.86 & 0.10 & 0.88 & 0.91\\
MICE & 0.03 & 0.03 & 0.03 & 0.03 & 0.30 & 0.31 & 0.30 & 0.29 & 0.29 & 0.29 & 0.09 & 0.94 & 0.94\\
TMLE & -0.37 & -0.15 & -0.18 & -0.16 & 3.48 & 1.09 & 0.86 & 0.82 & 0.85 & 0.85 & 0.18 & 0.85 & 0.89\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item Abbreviations: cOR: conditional odds ratio; Est: Estimator; Mn: Mean; Med: Median; WMn: Winsorized mean; TMn: trimmed mean; ESE: empirical standard error; MAD: median absolute deviation; ASE: asymptotic standard error; bias/SE: absolute Med bias / Med ASE; CP: coverage probability based on the ASE; CP*: coverage probability based on the ASE, where non-convergent datasets were dropped for all estimators; GR: generalized raking; IPW: inverse probability weighting; MICE: multiple imputation via chained equations; TMLE: targeted maximum likelihood estimation. Results are based on 2500 Monte-Carlo replications. 430 values were removed when computing GR performance due to non-convergence. Bolding indicates columns that we recommend using. The inverse square root of the effective sample size is 0.1.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> synthetic_simulation_results_cOR_n15000.tex <==
\begin{table}[!h]
\centering
\caption{Estimating the cOR in a rare-outcome, high missing-data setting, n = 15000.\label{tab:synthetic_results_cOR_n15000}}
\centering
\fontsize{8.5}{10.5}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{l>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.3in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}>{\raggedleft\arraybackslash}p{0.22in}}
\toprule
Est & Mn bias & \textbf{Med bias} & WMn bias & TMn bias & ESE & \textbf{MAD} & Mean ASE & \textbf{Med ASE} & WMn ASE & TMn ASE & bias / SE & CP & \textbf{CP*}\\
\midrule
GR & -0.01 & -0.01 & -0.01 & -0.01 & 0.76 & 0.31 & 0.29 & 0.27 & 0.29 & 0.28 & 0.03 & 0.83 & 0.92\\
IPW & -0.09 & -0.09 & -0.07 & -0.08 & 1.32 & 0.75 & 0.72 & 0.68 & 0.71 & 0.71 & 0.13 & 0.92 & 0.93\\
MICE & 0.01 & 0.02 & 0.01 & 0.01 & 0.24 & 0.24 & 0.24 & 0.24 & 0.24 & 0.24 & 0.07 & 0.96 & 0.96\\
TMLE & -0.10 & -0.09 & -0.09 & -0.09 & 1.36 & 0.81 & 0.72 & 0.68 & 0.71 & 0.71 & 0.12 & 0.90 & 0.91\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item Abbreviations: mOR: marginal odds ratio; Est: Estimator; Mn: Mean; Med: Median; WMn: Winsorized mean; TMn: trimmed mean; ESE: empirical standard error; MAD: median absolute deviation; ASE: asymptotic standard error; bias/SE: absolute Med bias / Med ASE; CP: coverage probability based on the ASE; CP*: coverage probability based on the ASE, where non-convergent datasets were dropped for all estimators; GR: generalized raking; IPW: inverse probability weighting; MICE: multiple imputation via chained equations; TMLE: targeted maximum likelihood estimation. Results are based on 2500 Monte-Carlo replications. 221 values were removed when computing GR performance due to non-convergence. Bolding indicates columns that we recommend using. The inverse square root of the effective sample size is 0.082.
\end{tablenotes}
\end{threeparttable}
\end{table}

